Extreme Regression for Dynamic Search Advertising

This paper introduces a new learning paradigm called eXtreme Regression (XR) whose objective is to accurately predict the numerical degrees of relevance of an extremely large number of labels to a data point. XR can provide elegant solutions to many large-scale ranking and recommendation applications including Dynamic Search Advertising (DSA). XR can learn more accurate models than the recently popular extreme classifiers which incorrectly assume strictly binary-valued label relevances. Traditional regression metrics which sum the errors over all the labels are unsuitable for XR problems since they could give extremely loose bounds for the label ranking quality. Also, the existing regression algorithms won't efficiently scale to millions of labels. This paper addresses these limitations through: (1) new evaluation metrics for XR which sum only the k largest regression errors; (2) a new algorithm called XReg which decomposes XR task into a hierarchy of much smaller regression problems thus leading to highly efficient training and prediction. This paper also introduces a (3) new labelwise prediction algorithm in XReg useful for DSA and other recommendation tasks. Experiments on benchmark datasets demonstrated that XReg can outperform the state-of-the-art extreme classifiers as well as large-scale regressors and rankers by up to 50% reduction in the new XR error metric, and up to 2% and 2.4% improvements in terms of the propensity-scored precision metric used in extreme classification and the click-through rate metric used in DSA respectively. Deployment of XReg on DSA in Bing resulted in a relative gain of 27% in query coverage. XReg's source code can be downloaded from http://manikvarma.org/code/XReg/download.html.

==> cache.tex <==
\iffalse
Although such regressors

Most of the conventional regression approaches~\citep{} learn a separate regressor for each outcome variable and hence do not scale to millions of labels present in XR scenarios. This problem is mitigated to some extent in the multi-objective decision tree based approaches~\citep{Kocev07,Agrawal13,Jain16} which scale sublinearly in the number on outcome variables. However, these approaches suffer from low accuracy despite learning a large ensemble of weak trees. 



Ranking and regression approaches are the natural alternatives for addressing the non-binary label relevance scenario. Given a data point, most ranking algorithms learn to rank a more relevant label higher than a less relevant label for each label pair. Since their training complexities scale quadratically in the number of labels $L$, they do not scale to millions of labels in DSA. On the other hand, the regression algorithms (sometimes called as pointwise rankers) predict a numerical score for each label that captures its relevance to a data point. These have $O(L)$ training and prediction time complexities, but still take weeks to train and several seconds to predict per test point, and hence do not meet the requirements of DSA. In comparison, \alg has $O(\log L)$ training and prediction time complexities and makes more relevant recommendations than the existing rankers and regressors.
\fi

-----

This paper proposes a new learning paradigm called Extreme Regression (XR) whose objective is to accurately predict the degrees of relevance of an extremely large number of labels with respect to a data point. XR can provide elegant solutions to many large-scale ranking and recommendation applications including Dynamic Search Advertising (DSA).

can be posed as the problem of estimating the click probabilities of millions of search queries with respect to each ad. These estimates can then be used to filter less clickable ads and re-rank the ads based on other models' estimates, advertiser bids {\it etc.} XR fixes a fundamental limitation of the recently popular extreme classification paradigm which assumes strictly binary-valued label relevances and hence learns less accurate models.


Based on these estimates, a small number of most clickable ads can be shown for a given query, usually after re-ranking steps to upvote the ads of high quality and high bids as well.

R can learn more accurate models than the recently popular extreme classification approaches which assume strictly binary-valued label relevances.

For example, Dynamic Search Advertising (DSA) can be posed as the problem of estimating the click probabilities of millions of search queries with respect to each ad. These estimates can be used to show a few, most clickable and highly bidded ads for a search query. XR remedies a fundamental limitation of the recently popular extreme classification paradigm which assumes strictly binary-valued label relevances and hence learns less accurate models. 

Traditional approaches to DSA based on information retrieval techniques~\citep{Jones00}, topic models~\citep{Wei06}, language models~\citep{Ravi10,Yih06} as well as deep learning~\citep{Huang13,Shen14} fail on pithy ad-landing pages or suffer from low query and ad coverages. Extreme classifiers such as Parabel~\citep{Prabhu18b} have also been applied to DSA with improved ad coverage and click-through rates, but their query coverage is low.

The objective of eXtreme Regression is to learn to accurately predict the real-valued, degrees of relevance of an extremely large number of labels with respect to a data point. Many large-scale ranking and recommendation applications can naturally be reformulated as XR problems. For example, DSA can be posed as an XR problem by treating millions of search queries as individual labels and predicting their click probabilities with respect to each ad (a data point). Similarly, the content-based movie recommendation task, involving millions of users (labels) and movies (data points), can be posed as the problem of predicting the user preferences over movies often in terms of discrete user ratings. The document tagging task involves estimating how well does each of a million tags (labels) describe a web document (data point). Here, a rare but specific tag is considered more informative than a popular but generic one, as quantified by the inverse propensity scores of these tags~\citep{Jain16}. These label relevance estimates can directly be used to recommend the most clickable ads, the most preferred movies or the most informative tags to a search query, a user or a document respectively. Additionally, these estimates also provide a principled way to improve the recommendations either by filtering off less relevant ones or by refining them further. For example, these estimates can be combined with the tail classifier scores from ~\citep{Jain16} to improve performance over really rare labels.

// ------------------

This paper introduces a new learning paradigm called eXtreme Regression (XR) whose objective is to accurately predict the real-valued degrees of relevance of an extremely large number of labels to a data point. These predictions could either be used to directly recommend a few, highly relevant labels to the data point or are consumed by further filtering and re-ranking steps. XR can provide elegant solutions to many large-scale ranking and recommendation applications including Dynamic Search Advertising (DSA). XR can learn more accurate models than the recently popular extreme classifiers which incorrectly assume strictly binary-valued label relevances. Traditional regression metrics which would sum the estimation errors over all the labels are unsuitable for XR problems where usually a small subset of labels need to be finally assigned to a data point. Furthermore, the existing regression algorithms won't efficiently scale to millions of labels. This paper addresses these limitations through: (1) {\it new evaluation metrics} for XR which measure the regression errors of only the most erroneous label relevance estimates; (2) a {\it new algorithm} called eXtreme Regressor (\alg\!) which decomposes XR problems into a hierarchy of much smaller regression problems thus leading to highly efficient training and prediction. This paper also introduces a (3) {\it new labelwise prediction algorithm} in \alg useful for DSA and other recommendation tasks.

Experiments on benchmark datasets demonstrated that \alg can outperform the state-of-the-art extreme classifiers as well as large-scale regressors and rankers by up to 2x, 2\% and 2.4\% in terms of the new XR metrics, the propensity-scored precision metrics used in extreme classification and click-through rate metric used in DSA respectively. Deployment of \alg on DSA in Bing resulted in a relative gain of 58\% in revenue and 27\% in query coverage. \alg's source code is available from \citep{XRegCode}.

would be necessary which could train and predict extremely efficiently in order to scale to millions of labels and data points while also maintaining high prediction accuracy. 

A few challenges arise while solving an XR problem. First, the algorithms need to . Second, the predicted relevances need to be highly accurate in order to 

enough to induce a good ranking 


most of the labels are 

where the end goal is to 

to ensure good recommendations both before and after the filtering and re-ranking steps.

-------------------


\iffalse
ir ranking. 

combining them with other algorithms' predictions. 

less relevant recommendations or to further refine them by combining with 

to refine the relevance 


These estimates are also useful in several downstream processing tasks such as: (1) label filtering based on relevance thresholds to obtain a favourable precision-recall trade-off; (2) combining these relevance weight estimates in a principled way with those from other approaches to improve accuracy further.

Such estimates can be used to directly 


The primary goal in these applications is to recommend a small number of most relevant labels for a data point. XR achieves this by estimating the relevance weights for each label and then recommending the top ranked labels according to these estimates. These estimates are also useful in several downstream processing tasks such as: (1) label filtering based on relevance thresholds to obtain a favourable precision-recall trade-off; (2) combining these relevance weight estimates in a principled way with those from other approaches to improve accuracy further. Hence, the predictions need to be accurate in terms of both ranking and regression performance. For faithful evaluation in such settings, the newly proposed XR metrics are more suitable than the existing regression or ranking metrics.


but relevant tag is 

when the total tags could range in millions. 

the descriptive abilities of millions of tags  a web page where rare tags are much more useful

Similarly, XR can also be used to predict the ratings that a user might give to new movies and thus recommend the most relevant movies.

Extreme classification itself can be posed as an XR problem of predicting the label relevance weights, generated as binary label relevances multiplied by the inverse propensity scores of respective labels, for a given data point. The inverse propensity scores give larger weights to rare labels which are often more useful~\citep{Jain16}. Similarly, XR can also be used to predict the ratings that a user might give to new movies and thus recommend the most relevant movies. DSA can also be posed as an XR problem. 
\fi


--------

{\bf Extreme Classification}: Extreme classifiers annotate a data point with the most relevant subset of labels from an extremely large label set. The state-of-the-art extreme classifiers such as Parabel~\citep{Prabhu18b} and Slice~\citep{Jain19} are able to train from millions of data points and labels in just a few hours and predict in just a few milliseconds per test point. This makes them appealing for really large-scale recommendation and ranking problems such as DSA~\citep{Prabhu18b}. Unfortunately, extreme classifiers make a fundamentally incorrect assumption that a label is either fully relevant or fully irrelevant to a data point. When applied to DSA, they approximate the real-valued click-through rates to 0 or 1 during training and thus end up predicting less clickable ads during prediction. In contrast, the proposed \alg algorithm extends the Parabel classifier to directly model these non-binary click probabilities, thus improving prediction accuracy while maintaining Parabel's high training and prediction efficiency. Note that whereas some extreme classifiers such as PfastreXML~\citep{Jain16} and LEML~\citep{Yu14} can be trivially modified to learn from real-valued relevances, they nevertheless suffer from low efficiency and low accuracy.


--------

To avoid these pitfalls, some works in advertising~\citep{Sculley10} evaluate performance using 2 different metrics for regression and ranking, but then simultaneously optimizing for multiple metrics is non-trivial. In comparison, the new XR metrics simultaneously minimize both ranking and regression error and are amenable to efficient optimization.


--------

\iffalse
This paper generalizes the precision@$k$ and nDCG@$k$ metrics traditionally used in extreme classification to {\it relevance-weighted} precision@$k$ and nDCG@$k$ which are defined, for a data point $i$, as follows:\vspace{-1mm}
\begin{align}
\text{WP@}k(\hat{\v y}_i,\v y_i) &= \frac{1}{k}\sum_{l \in S(\hat{\v y}_i,k)} y_{il}\\
\text{WN@}k(\hat{\v y}_i,\v y_i) &= \frac{1}{iDCG(\v y_i)}\sum_{l \in S(\hat{\v y}_i,k)} \frac{y_{il}}{\log_2(l+1)}
\end{align}
where $iDCG(\v y_i)$ is a standard normalizer which ensures that WN@$k$ always lies between $0$ and $1$~\citep{Jarvelin02}. They measure the quality of ranking only in the top $k$ positions and also take into account the degree of label relevances. The WP@$k$ metric reduces to (a) PSP@$k$ when $\v y_i$ are set to inverse propensity-scores multiplied by binary relevances; (b) CTR@$k$ suitable for DSA when $\v y_i$ is set to the ad click-through rates; (c) Rating@$k$ when $\v y_i$ is set to the user ratings, which is the undiscounted version of the familiar rating-based nDCG@$k$ metric used in recommender systems~\citep{Jarvelin02}.

Beside these, we also report using the AUC@$k$ metric which is widely used in recommendation and ranking literature~\citep{Lee14}:
\begin{align}
\text{AUC@}k( \hat{\v y}_i,\v y_i) &= 1 - \frac{1}{|M(\v y_i)|} \sum_{\substack{(l,l') \in M(\v y_i)\\l \in S(\hat{\v y}_i,k)}} \mathbb{I}[\hat{y}_{il}>\hat{y}_{il'}]
\end{align}
This metric measures the number of wrongly ordered label pairs in terms of their relevance weights with $M(\v y_i)$ being the maximum number of such pairs.
\fi


------

Although the above metrics are useful for measuring the ranking accuracy, they fully ignore the regression performance necessary for XR applications. To address this limitation, we introduce novel XR error metrics. which could be used to simultaneously minimize the ranking and regression errors in the top $k$ ranks:
\begin{align}
    &\text{Ranking-error@}k(\hat{\v y}_i,\v y_i) = \frac{1}{k}\sum_{l \in S(\v y_i,k)} y_{il} - \frac{1}{k}\sum_{l \in S(\hat{\v y}_i,k)} y_{il} \\
    &\text{Regression-error@}k(\hat{\v y}_i,\v y_i) = \frac{1}{k}\sum_{l \in S(\hat{\v y}_i,k)} |\hat{y}_{il}-y_{il}|
\end{align}

-----

\iffalse
\begin{proof}
The proof is available in the \suppurl.
\end{proof}\vspace{-0.5mm}
\fi

-----

%Furthermore, \alg is highly efficient with $O(\text{polylog}(L))$ computational and sample complexities in the number of labels $L$ and thus easily scales large datasets with millions of labels. 
% @Yash, second para of abstract makes no sens if we remove the words PSP, CTR and XMAD


-----

DSA can be posed as an XR problem by treating the millions of search queries as individual labels and predicting their click probabilities with respect to each ad (a data point). Similarly, the movie recommendation and document tagging tasks can also be posed as XR problems of predicting, respectively, the ratings of movies given by millions of users and the informativeness of millions of tags for describing a web document. Based on such relevance estimates, the most clickable ads, the most preferred movies or the most informative tags can be recommended to a search query, a user or a document respectively. Additionally, these estimates also provide a principled way to further refine the recommendation set by either filtering off less relevant ones or by re-ranking them. An example of re-ranking is to combine these estimates with the scores from tail classifiers~\citep{Jain16} to improve the recommendation accuracies over rare labels. To successfully solve an XR problem, new algorithms which could train and predict efficiently on millions of labels and data points while also maintaining high prediction accuracy are required. Furthermore, the definition of accuracy, or equivalently regression error, needs to be redefined for XR settings where both the relevant labels and the desired label recommendations are extremely small in number compared to the complete label set whose most labels have no influence on final recommendations. This paper addresses these challenges by developing new evaluation metrics and algorithms.

-----

by using the observation that most labels in XR applications are fully irrelevant to a data point. \alg achieves this by leveraging a balanced label tree which partitions the relevant labels together for most data points. Due to this, large groups of fully irrelevant labels frequently occur for which common regressors can be learnt, thus leading to highly efficient training. During prediction, a data point greedily traverses the label tree by exploring only logarithmic number of most promising paths which lead to highly relevant labels. The \alg method is similar to Parabel in many ways. However, unlike Parabel, the tree construction uses non-binary relevance weights leading to better partitions, the nodes contain efficient regressors instead of classifiers, and the predictions give reliable relevance weight estimates along with label rankings. As a result, \alg can be up to 3\% better in relevance-weighted precision and 2x better in XR metrics than Parabel. \alg also consistently outperforms large-scale regressors and rankers in terms of both regression and ranking errors.

==> metrics.tex <==
\begin{table*}[]
\centering
\captionsetup{font=small}
	\caption{Enter caption.}
	\label{tab:madvsxmad}
	\begin{minipage}[t]{0.5\linewidth}
		\resizebox{\linewidth}{!}
		{
\begin{tabular}{@{}lccccc@{}}
\toprule
Method & \begin{tabular}[c]{@{}c@{}}WP@5\end{tabular}    & \begin{tabular}[c]{@{}c@{}}WP-t@5\end{tabular}      & MAD             & \begin{tabular}[c]{@{}c@{}}MAD-t / \\XMAD@5\end{tabular} & XMAD-t@5 & AUC-pr  \midrule
\multicolumn{6}{c}{EURLex-4K}                                                                                                                                                         \\ \midrule
PfastreXML                 & 0.1356          & 0.4091          & 2.5309          & 3.02                                                                 & 6.19                                                        \\
Parabel                    & 0.1436          & 0.4345          & 3.0574          & 3.03                                                                 & 7.04                                                        \\
LEML                       & 0.1468          & 0.5210          & 6.2443          & 3.55                                                                 & 11.99                                                       \\
1-vs-all-LS                & \textbf{0.1342} & 0.4736          & 14.7169         & 3.53                                                                 & 31.07                                                       \\
RankSVM                    & 0.1377          & 1.2224          & 37.7822         & 8.88                                                                 & 30.91                                                       \\
DiSMEC                     & 0.1607          & 0.4163          & 46.9473         & \textbf{2.59}                                                        & 112.77                                                      \\
\alg        & 0.1394          & \textbf{0.3957} & \textbf{2.1915} & 2.84                                                                 & \textbf{5.54}                                               \\
\alg-t      & 0.1389          & 0.4906          & 5.9701          & 3.53                                                                 & 12.17                                                       \\ \midrule
\multicolumn{6}{c}{Wiki10-31K}                                                                                                                                                                                        \\ \midrule
PfastreXML                 & 0.4861          & 0.8862          & 9.3561          & 1.82                                                                 & 10.56                                                       \\
Parabel                    & 0.4990          & 1.1784          & 10.1523         & 2.36                                                                 & 8.62                                                        \\
LEML                       & 0.5027          & 0.8886          & 25.5622         & \textbf{1.77}                                                        & 28.77                                                       \\
1-vs-all-LS                & 0.4515          & \textbf{0.8492} & 34.1409         & 1.88                                                                 & 40.20                                                       \\
RankSVM                    & 0.4714          & 2.2960          & 75.4734         & 4.87                                                                 & 32.87                                                       \\
DiSMEC                     & 0.4878          & 1.1519          & 80.3084         & 2.36                                                                 & 69.72                                                       \\
\alg        & 0.4802          & 0.8938          & \textbf{6.0104} & 1.86                                                                 & \textbf{6.72}                                               \\
\alg-t      & \textbf{0.4475} & 0.8741          & 32.2013         & 1.95                                                                 & 36.84                                                       \\ \bottomrule
\end{tabular}
		}
		\end{minipage}%
		\begin{minipage}[t]{0.5\linewidth}
		\resizebox{\linewidth}{!}
		{
\begin{tabular}{@{}lccccc@{}}
\toprule
Method & \begin{tabular}[c]{@{}c@{}}WP-regret-l\\ @k\end{tabular}    & \begin{tabular}[c]{@{}c@{}}2*XMAD-l\\ @2k\end{tabular}      & MAD             & \begin{tabular}[c]{@{}c@{}}2*XMAD-l@2k / \\WP-regret-l@k\end{tabular} & \begin{tabular}[c]{@{}c@{}}MAD /\\ WP-regret-l@k\end{tabular} \\ \midrule
\multicolumn{6}{c}{YahooMovie-8K}                                                                                                                                                                                     \\ \midrule
PfastreXML                 & 0.5665          & 0.8875          & 8.4893          & 1.57                                                                 & 9.57                                                        \\
Parabel                    & 0.5693          & 0.8850          & \textbf{6.3913} & \textbf{1.55}                                                        & \textbf{7.22}                                               \\
LEML                       & 0.4933          & 0.9571          & 36.0738         & 1.94                                                                 & 37.69                                                       \\
1-vs-all-LS                        & 0.4943          & 0.9288          & 47.1887         & 1.88                                                                 & 50.81                                                       \\
RankSVM                    & 0.4738          & 2.0235          & 76.6099         & 4.27                                                                 & 37.86                                                       \\
DiSMEC                     & 0.4760          & 0.9003          & 38.0254         & 1.89                                                                 & 42.24                                                       \\
XLR                        & 0.6013          & 1.0423          & 17.0795         & 1.73                                                                 & 16.39                                                       \\
\alg       & 0.4676          & \textbf{0.8847} & 6.7809          & 1.89                                                                 & 7.66                                                        \\
\alg-t      & \textbf{0.4664} & 0.8964          & 12.1071         & 1.92                                                                 & 13.51                                                       \\ \midrule
\multicolumn{6}{c}{DSA-130K}                                                                                                                                                                                          \\ \midrule
PfastreXML                 & 0.0289          & 0.0500          & 0.3291          & 1.73                                                                 & 6.58                                                        \\
Parabel                    & 0.0266          & 0.1230          & 0.8827          & 4.62                                                                 & 7.18                                                        \\
LEML                       & 0.0361          & \textbf{0.0486} & 0.2828          & \textbf{1.35}                                                        & 5.82                                                        \\
DiSMEC                     & 0.0265	       & 0.1547             &	4.0878 & 5.84&26.42\\
XLR                        & 0.0402          & 0.9157          & 34.429          & 22.78                                                                & 37.60                                                       \\
\alg       & 0.0259          & 0.0519          & \textbf{0.2482} & 2.00                                                                 & \textbf{4.78}                                               \\
\alg-t      & \textbf{0.0256} & 0.0787          & 0.5862          & 3.07                                                                 & 7.45                                                        \\ \bottomrule
\end{tabular}
		}
		\end{minipage}
		\vspace{-2mm}
\end{table*}



==> pspcomp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t!]
\centering
\captionsetup{font=small}
		\caption{Comparison of Propensity Scored Precision@$k$ (PSP@$k$) in (\%) for $k=1, 3, 5$ for \alg against the state-of-art extreme classifiers DiSMEC and ProXML where \alg consistently outperforms them across 5 pointwise datasets from the Extreme Classification Repository.}
		\label{tab:pspcomp}
\resizebox{\linewidth}{!}
  {
\begin{tabular}{@{}cccccccccccccccc@{}}
\toprule

\multicolumn{1}{l|}{Method}              & PSP@1 & PSP@3 & \multicolumn{1}{c|}{PSP@$5$} & PSP@1 & PSP@3 & \multicolumn{1}{c|}{PSP@$5$} & PSP@1 & PSP@3 & \multicolumn{1}{c|}{PSP@$5$} & PSP@1 & PSP@3 & \multicolumn{1}{c|}{PSP@$5$} & PSP@1     & PSP@3    & PSP@$5$    \\ \midrule                                   & \multicolumn{3}{c}{BibTeX-p}                 & \multicolumn{3}{c}{EURLex-4K-p}              & \multicolumn{3}{c}{Wiki10-31K-p}             & \multicolumn{3}{c}{WikiLSHTC-325K-p}         & \multicolumn{3}{c}{Amazon-670K-p} \\ \midrule
\multicolumn{1}{l|}{\alg} & 49.86 & \textbf{53.04} & \multicolumn{1}{c|}{\textbf{58.77}} & \textbf{45.23} & \textbf{48.51} & \multicolumn{1}{c|}{\textbf{51.39}} & \textbf{25.92} &\textbf{ 23.56} & \multicolumn{1}{c|}{\textbf{22.60}} & \textbf{36.85} & \textbf{37.98} & \multicolumn{1}{c|}{40.33} & \textbf{31.29}     & \textbf{32.89}    & 34.42    \\
\multicolumn{1}{l|}{ProXML}              & \textbf{50.10} & 52.00 & \multicolumn{1}{c|}{58.30} & 45.20 & 48.50 & \multicolumn{1}{c|}{51.00} & -     & -     & \multicolumn{1}{c|}{-}     & 34.80 & 37.70 & \multicolumn{1}{c|}{\textbf{41.00}} & 30.80     & 32.80    & \textbf{35.10}   \\
\multicolumn{1}{l|}{DiSMEC}              & -     & -     & \multicolumn{1}{c|}{-}     & 41.20 & 45.40 & \multicolumn{1}{c|}{49.30} & 13.60 & 13.10 & \multicolumn{1}{c|}{13.80} & 29.10 & 35.60 & \multicolumn{1}{c|}{39.50} & 27.80      & 30.60     & 34.20     \\ \bottomrule
\end{tabular}
}
\end{table}
